Sampling-based Model Predictive Control Leveraging Parallelizable Physics Simulations

We present a method for sampling-based model predictive control that makes use of a generic physics simulator as the dynamical model. In particular, we propose a Model Predictive Path Integral controller (MPPI), that uses the GPU-parallelizable IsaacGym simulator to compute the forward dynamics of a problem. By doing so, we eliminate the need for explicit encoding of robot dynamics and contacts with objects for MPPI. Since no explicit dynamic modeling is required, our method is easily extendable to different objects and robots and allows one to solve complex navigation and contact-rich tasks. We demonstrate the effectiveness of this method in several simulated and real-world settings, among which mobile navigation with collision avoidance, non-prehensile manipulation, and whole-body control for high-dimensional configuration spaces. This method is a powerful and accessible open-source tool to solve a large variety of contact-rich motion planning tasks.

==> tex/related_work.tex <==
\section{Related work}
\label{sec:related_work}
In this section, we present a selected collection of works, with a particular focus on motion planning and contact-rich tasks. 
Motion planning pipelines can be roughly split into global and local motion planning \cite{siegwart2011introduction}. 
Global motion planning ensures globally feasible paths considering a snapshot of the entire environment at planning 
time. Such methods include classical grid-based approaches, such as A*, and configuration space sampling methods, 
such as rapidly exploring random trees (RRT) and probabilistic roadmaps (PRM), \cite{karaman2011sampling}. 
As we propose a method for contact-rich tasks, we do not further discuss global planning methods.
In dynamic environments, global planning methods are paired with local planning methods, also referred to as trajectory
generation methods. Approaches for local motion planning range from control methods, such as operational space control, and geometric approaches, such as Riemannian Motion Policies \cite{li2022multi} and Optimization Fabrics \cite{ratliff2021generalized,spahn2023dynamic}, to receding-horizon optimization formulations \cite{avanzini2018constrained}, potentially combined with learned components \cite{hewing2020learning}.
\MS{Not sure about the transition, yet}

% Conventional MPC
MPC is one of the most popular popular techniques \cite{schwenzer2021review}. Most MPC algorithms are based on constrained optimization techniques that assume smooth dynamics to solve the motion planning problem. Thus, one has to come up with clever ways to solve the optimization in real-time and rely on extensive modeling to complete an otherwise simple pushing task~\cite{hogan_reactive_2020, moura_non-prehensile_2022}.
In fact, in the context of contact-rich tasks pose a challenge to current methods, due to their non-smooth and hybrid nature, such as transitioning from sticking to sliding motion or entering a contact. 
 
%Instead of relying on accurate modeling, \cite{toussaint2022sequence} proposes an MPC approach dedicated to robustly executing a single sequence of constraints by planning for timing-optimal transitions among them. This leads to frequent re-initiation behaviors, which in turn, however, compensates for inaccurate models. 

% Sampling MPC
In contrast, Model Predictive Path Integral (MPPI) control~\cite{Williams2017c, williams_information-theoretic_2018} are sampling-based MPCs, a class of algorithms that rely on parallel sampling of input sequences to approximate the optimal control. This characteristic makes these algorithms gradient-free and therefore suitable for systems with non-linear discontinuous dynamics and cost functions. MPPI is a promising direction because derivative information is not required, thus one can tackle tasks with non-smooth and discontinuous dynamics. In addition, similar to other sampling-based strategies, MPPI is easily parallelizable.

MPPI has been shown to be capable of controlling a high-degrees of freedom manipulator in real-time~\cite{bhardwaj_storm_2021}. Self-collision avoidance is achieved by using a trained neural network and a learned collision-checking function from \cite{danielczuk2021object} that uses point clouds directly. Even though this allows for real-time control, additional learned models for collision avoidance are required, and interaction with objects the environment is not possible.

In \cite{abraham2020model}, the authors propose an online ensemble MPPI that completes complex tasks while being adaptive to parameter
uncertainty. However, the modeling of the tasks remains unclear no open-source implementation is provided.

To alleviate the problem of explicit modeling, there have been a handful of previous attempts which proposed the use of physics simulators for sampling-based MPC, however, they present some limitations.
In recent work~\cite{howell_predictive_2022}, a simple sampling-based MPC has been proposed which relies on a physics engine, namely MuJoCo~\cite{todorov_mujoco_2012}, as a dynamic model of the environment for rolling out the sampled input sequences. By doing so, the motion planner offloads all of the modeling efforts to the physics engine, vastly simplifying the controller design.
Despite its fast computation, MuJoCo's parallelization capabilities are bounded by the number of threads of the CPU, which limits the number of environments one can sample in parallel to achieve real-time performances.
In \cite{carius2022constrained} Raisim only some waypoints for foot placement are sampled. With our method, we can compute a control policy on the fly even for high DOFs systems.

% Contact rich literature
In this work, we focus on non-prehensile manipulation and picking tasks that require contact with a variety of objects. 

Non-prehensile manipulation with robot arms is usually limited to the sampling of end-effector trajectories on a plane, relying on additional controllers to ultimately actuate the robot. For instance, Arruda et al. \cite{arruda2017uncertainty} utilize a forward-learned model trained on 326 real robot pushes. This model is employed by an MPPI controller to plan push manipulations as end-effector trajectories. Inverse kinematic solvers are then used to find solutions and control the robot. The push manipulation task is accomplished through a sequence of pushes, with re-initialization during execution. Cong et al. \cite{cong2020self} train an LSTM-based model to capture push dynamics using a dataset of 300 randomized objects. End-effector trajectories are sampled within a rectangular 2-D workspace above the table, maintaining an upright stick position. A separate controller converts Cartesian end-effector motions into joint commands. The push task involves a sequence of pushes, resulting in discontinuous motion. The LSTM model requires multiple warm-up steps for reliable predictions.
Finally, these methods are not easily transferrable for instance to non-differential drive mobile pushing. 

% Summarize problems in the literature and contributions
In this paper, we propose a general method to tackle motion planning in contact-rich tasks. No need to train specialized models of control policies, as well as no need for additional inverse kinematic solvers or controllers. Instead, we directly sample control inputs and use generic physics as a dynamic model. This allows for cheap collision checking and prediction of robot-object and object-object interactions for free. To summarize, the contributions of our work are the following:
\begin{itemize}
    \item A general way of solving sampling-based MPC where the dynamical model is a physics simulator.
    \item An open-source implementation that is easy to extend to new robots, tasks, and environments.
\end{itemize}

We showcase how with the same strategy we can tackle different tasks, including mobile navigation, non-prehensile manipulation, and whole-body control for mobile manipulation. We benchmark the solution against recent methods and outperform them in most tasks. We also analyze the benefits and limitations of our approach, openly acknowledging its main challenges and directions for future work. 

% 
% Also have a read at [\href{https://repository.tudelft.nl/islandora/object/uuid\%3Adfbb72de-5abe-4cf8-bb7a-b1d278ea6b78?collection=education}{this}].

%The emergence of these behaviors extends also to tasks that are notoriously hard from both a classical control as well as a learning perspective. Similarly to \cite{howell2022predictive}, in fact, we show how one can synthesize online complex manipulation skills such as cube re-arranging with the shadow hand, without any learning.

